Better Safe than Sorry: Recovering after Adversarial Majority

The security of blockchain protocols is a combination of two properties: safety and liveness. It is well known that no blockchain protocol can provide both to sleepy (intermittently online) clients under adversarial majority. However, safety is more critical in that a single safety violation can cause users to lose money. At the same time, liveness must not be lost forever. We show that, in a synchronous network, it is possible to maintain safety for all clients even during adversarial majority, and recover liveness after honest majority is restored. Our solution takes the form of a recovery gadget that can be applied to any protocol with certificates (such as HotStuff, Streamlet, Tendermint, and their variants).

==> lib/spacinghacks.tex <==
%
%
%
%

%
%
%
%

%
%
%
%

%
%

%
%
%
%
%
%
%
\widowpenalty=0
\clubpenalty=0
\brokenpenalty=0
%

%
%
%

%
%
%
%
%


